Hyperbolic Components

Consider polynomial maps $f:\C\to\C$ of degree $d\ge 2$, or more generally polynomial maps from a finite union of copies of $\C$ to itself. In the space of suitably normalized maps of this type, the hyperbolic maps form an open set called the hyperbolic locus. The various connected components of this hyperbolic locus are called hyperbolic components, and those hyperbolic components with compact closure (or equivalently those contained in the "connectedness locus") are called bounded hyperbolic components. It is shown that each bounded hyperbolic component is a topological cell containing a unique post-critically finite map called its center point. For each degree $d$, the bounded hyperbolic components can be separated into finitely many distinct types, each of which is characterized by a suitable reduced mapping scheme $\bar S_f$. Any two components with the same reduced mapping scheme are canonically biholomorphic to each other. There are similar statementsfor real polynomial maps, for polynomial maps with marked critical points, and for rational maps. Appendix A, by Alfredo Poirier, proves that every reduced mapping scheme can be represented by some classical hyperbolic component, made up of polynomial maps of $\C$. This paper is a revised version of [M2], which was circulated but not published in 1992.

==> milnor-A.tex <==
\section{Realizing Reduced Schemes (by Alfredo Poirier\protect\footnotemark[6])\label{sa}}   %%%% aug 29, 2011 
\bigskip

The purpose of this appendix is to prove that every reduced mapping scheme can
 be realized by a postcritically finite polynomial. 
In order to do so, we will construct an appropriate Hubbard tree that mimics 
the dynamics of the scheme. 
For the benefit of the reader we recall briefly the main concepts involved in 
the construction of Hubbard trees  following closely \cite{P3}.\medskip  


\footnotetext[6]
{Departmento de Ciencias, Secci\'on Matem\'aticas, Pontificia Universidad Cat\'olica del Per\'u, Apartado 1761, Lima 100, Per\'u;  \hspace{.5cm}
{\it email\/}: {apoirie@pucp.edu.pe}}
\setcounter{footnote}{6}

Given a degree $d \ge 2$ postcritically finite polynomial $f$, 
we know that its \textbf{\textit{filled Julia set}} $K(f)$, besides being 
connected, is locally connected.  Call a periodic orbit that contains a 
critical point a \textbf{\textit{critical cycle}}. 
In the postcritically finite setting, a periodic orbit belongs to the Fatou 
set $F(f)$ if and only if it is a critical cycle 
(for details we refer to \cite[Corollary 14.5]{M4}). 

In this postcritically finite case, the polynomial $f$ when restricted to the 
interior of $K(f)$ 
(which happens to be nonempty only when there exists a critical cycle) 
maps each bounded Fatou component 
---always simply connected by the maximum modulus principle--- 
onto some other as a branched covering map. 
Furthermore, all of them are eventually periodic (see \cite[Theorem 16.4]{M4}). 
And also, each component can be uniformized so that in local charts 
$f$ reads $z \mapsto z^m$ for some $m \ge 1$ (see \cite[Theorem 9.1]{M4}). 
More is true. 
If $U$ is a periodic bounded Fatou component, 
then the first return map is conjugate to $z \mapsto z^k$, this time with 
$k \ge 2$. 
In particular, loops of components are in perfect correspondence with critical
 cycles. 
Also, in each component there is a unique point which eventually maps to a 
critical point 
(precisely the one marked as $0$ in local coordinates), its 
\textbf{\textit{center}}. 

It is well known (see for instance \cite[Corollary VII.4.2]{DH1}) 
that given a degree $d \ge 2$ postcritically finite polynomial $f$,  
for any $z \in K(f)$ the sets $K(f)-\{z\}$ and $J(f)-\{z\}$ consist both of a 
finite number of connected components.  
In this way, the filled Julia set can be thought of as arranged in a tree-like
 fashion. 

To get rid of inessentials, we pick a finite invariant set $M$ containing all 
critical points. 
Within $K(f)$ we interconnect $M$ by arcs subject to the extra condition that 
when a Fatou component is met, 
then this intersection consists of radial segments in the associated 
coordinate. 
Douady and Hubbard proved that this construction defines a finite topological 
tree $T(M)$ 
when $M$ together with the intrinsic branching points are considered vertices. 

The vertex dynamics is invariant and carries the endpoints of any edge to 
distinct elements, 
so that it can be extended to a function from $T(M)$ to itself which is one to
 one on each edge 
and is isotopic to $f$, the original map. 
We also keep record of the local degree at every vertex $v$ as $d(v)$. 
In addition, if three or more edges meet at a vertex, 
then their cyclic order should be remembered. 
In other words, we specify how this tree is embedded in the complex plane, 
again, up to isotopy. 

Unfortunately, this data alone is not enough to determine the affine conjugacy
 class of $f$. 
However, if we append enough information to recover the inverse tree, 
then different postcritically finite polynomials yield different structures. 
To formally deal with this condition we introduce angles around vertices 
(this is to be credited again to \cite{DH1}). 
In what follows we measure angles in turns, so that 1 degree measures 1/360 of
 a turn. 
At the center of a component the angle between edges is measured using the 
local chart. 
Near Julia vertices, where $m$ components of $K(f)$ intersect, 
the angle is naturally defined as a multiple of $1/m$. 

These angles satisfy two obvious conditions. 
First, they are compatible with the embedding of the tree. That is, as we
go around a vertex in the positive direction, the successive angles are between
zero and one, and add up to $+1$. Second, they satisfy the identity 
$$
\angle_{f(v)}(f(e),f(e'))=d(v)\angle_{v}(e,e') \mod 1,
$$ 
where $d(v)$ is the local degree at $v$, and $e,e'$ are edges incident at $v$. 
When this further structure is provided, 
we are in front of a \textbf{\textit{Hubbard tree}}. 

\subsection*{Abstract Hubbard Trees}
Now we move in reverse: 
we start with an abstract dynamical tree and we reconstruct the appropriate 
postcritically finite polynomial.

An \textbf{\textit{angled tree $H$}} is a finite simplicial tree  
together with a function\break $e,e' \mapsto \angle_{v}(e,e') \in \mathbb Q/ 
\mathbb Z$ 
which assigns a rational number modulo $1$ to each pair of edges $e,e'$ 
incident at a vertex $v$. 
The \textbf{\textit{angle}} $\angle_{v}(e,e')$ is skew symmetric 
with $\angle_{v}(e,e')=0$ if and only if $e=e'$, 
and satisfies $\angle_{v}(e,e'')=\angle_{v}(e,e')+\angle_{v}(e',e'')$ 
whenever the three edges meet at $v$.  This angle function 
 determines a preferred isotopy 
class of embeddings of $H$ into $\mathbb C$. 

Let $V$ be the set of vertices in $H$.  We specify a 
\textbf{\textit{vertex dynamics}} $f:V \to V$ subject to $f(v) \ne f(v')$ 
whenever $v,v'$ are  end-points of a common %contiguous throughout an
 edge $e$. 
We consider also a \textbf{\textit{local degree}} 
\hbox{$d:V \to  \{1,2,\dots\}$}. We require that the 
\textbf{\textit{total degree}} \hbox{$d_H=1 + \sum_{v \in V} (d(v)-1)$} must be
 greater than $1$.  By definition a vertex is \textbf{\textit{critical}} if 
$d(v)>1$ and non-critical otherwise.  The \textbf{\textit{critical set}} is 
thus non-empty.  

We require $f$ and the degree $d$ to be related to the angles 
 as follows. 
Extend $f$ to a map \hbox{$f:H \to H$} that carries each edge homeomorphically
 onto 
the shortest path joining the images of its endpoints. We  then need
\hbox{$\angle_{f(v)}(f(e),f(e'))=d(v)\angle_{v}(e,e')$} whenever $e,\, e'$ are 
incident at $v$ 
(so that $f(e),\, f(e')$ intersect at the vertex $f(v)$
 where the angle is measured). 

A vertex $v$ is \textbf{\textit{periodic}} if \hbox{$f^{\circ k}(v)=v$} for some 
\hbox{$k \ge 1$}.  The orbit of a periodic critical point is a 
\textbf{\textit{critical cycle}}.  A vertex is of \textbf{\textit{Fatou type}}
 if it eventually maps to a critical cycle;  else, it is of 
\textbf{\textit{Julia type}} or a \textbf{\textit{Julia vertex}}. 

The distance \hbox{$dist_{H}(v,v')$} between vertices in $H$ counts the number
 of  edges in the shortest path joining $v$ to $v'$.  We call $H$ 
\textbf{\textit{expanding}} if for every edge $e$ whose endpoints $v,v'$ are 
Julia vertices  there is $n \ge 1$ for which we have 
$$dist_{H}(f^{\circ n}(v),f^{\circ n}(v')) > 1.$$ 
(In practice this property must be tested only for adjacent Julia vertices.)

Angles at Julia vertices are rather artificial, so it is better to normalize 
them.  
If $m$ edges \hbox{$e_1,\,\dots,\,e_m$} meet at a periodic Julia vertex $v$, 
then each \hbox{$\angle_{v}(e_i,e_j)$} should be a multiple of $1/m$. 
(Therefore, angles around a periodic Julia vertex convey no information beyond
 the cyclic order of the edges.) 
An angled tree that satisfies this 
 condition around all periodic Julia vertices
 is said to be \textbf{\textit{normalized}}. 

By an \textbf{\textit{abstract Hubbard tree}} ---or simply a Hubbard tree--- 
we mean a normalized angled tree that obeys the expanding condition. 
The basic existence and uniqueness theorem is stated now as follows.
\medskip 
 
\begin{theorem}[Poirier \cite{P3}]\label{t-A1P}
A normalized dynamical angled tree can be realized as the tree associated to a 
postcritically finite polynomial if and only if it is expanding,
or in other words if and only if it is an abstract Hubbard tree. 
Such a realization is unique up to affine conjugation. 
\end{theorem}

Note that there many cases where we can apply this result directly: 
any tree which has no adjacent Julia vertices is trivially expanding. 
For instance, a star-shaped dynamical tree in which a critical cycle
 pivots around a fixed vertex can always be realized. 
\medskip 

Now we are ready to realize a given reduced scheme \hbox{$\overline{S}=(
|\overline{S}|,\, F,\, \w)$} and  
settle the existence of a postcritically finite polynomial $f$ of degree 
\hbox{$d(\overline{S})=\w(\overline{S})+1$}
whose associated reduced scheme \hbox{$\overline{S}(f)$} is isomorphic to
$\overline{S}$. 

\begin{theorem} 
Every reduced scheme can be  realized by a postcritically finite polynomial.
\end{theorem} 

\begin{proof}
First we construct a non-reduced scheme $S$ which reduces to $\overline{S}$. 
This is done by adding new vertices of weight zero 
in such a way that the associated graph $\Gamma(S)$ can be obtained from 
\hbox{$\Gamma(\overline{S})$}
by plotting an extra vertex within each old edge.
(Compare Figures \ref{f-A.1} and \ref{f-A.2}, where the new vertices are 
indicated by small circles.)
More explicitly, 
starting with a reduced scheme $\overline{S}$ with associated map 
$\overline{F}:|\overline{S}| \to |\overline{S}|$, 
construct a non-reduced scheme $S$ with associated map $F:|S| \to |S|$, where
 $|\overline{S}| \subset |S|$, as follows. 
The difference set $|S|-|\overline{S}|$ is to consist of one vertex 
$s^{\sharp}$ for each $s \in |\overline{S}|$, and the map $F:|S| \to |S|$ is 
defined by
$$
F(s)=s^{\sharp} \qquad \hbox{and} \qquad 
F(s^\sharp)=s', \qquad \hbox{where} \qquad s'=\overline{F}(s). 
$$

\begin{figure}[!ht]
\centerline{\psfig{figure=milnor-fig11.eps,height=.8in}}
\vspace{-.4cm}
\caption{\it \label{f-A.1} A reduced scheme.}
\bigskip

\end{figure}


\begin{figure}[!ht]
\bigskip

\centerline{\psfig{figure=milnor-fig12.eps,height=.8in}}
\caption{\it \label{f-A.2} The associated non reduced mapping scheme. 
From each cycle we pick a representative ($c_1,\,c_2$). 
All non-periodic critical points are also named ($c_3,\,c_4$).}
\end{figure}

In simple words, $s^{\sharp}$ lies in the middle of $s$ and 
$s'=\overline{F}(s)$, 
so that the main difference between $F$ and $\overline{F}$ is that a vertex 
$s \in |\overline{S}|$ 
now takes an intermediate (artificial) step before reaching 
$s'=F(s) \in |\overline{S}|$. 
Formally, we have $F^{\circ 2}=\overline{F}$ when restricted to 
$|\overline{S}|$. 

By its very definition, every vertex of the form $s^\sharp$ has $s$ as its only 
preimage. 
From this construction it follows readily that $S$ has $\overline{S}$ as its
reduced scheme. 
This scheme is the one that we will bring to life with the help of a suitable 
expanding Hubbard tree. 

\begin{figure}[!ht]
\centerline{\psfig{figure=milnor-fig13.eps,height=1.5in}}
\caption{\it \label{f-A.3} The dynamical graphs corresponding to the two 
cycles in Figure \ref{f-A.2}.}
\end{figure}

Let ${\mathcal C}_i$ be a cycle 
$s_0 \mapsto s_0^{\sharp} \mapsto s_{1} \mapsto \cdots \mapsto s_{n-1}^{\sharp} 
\mapsto s_{0}$ in $S$. 
We join all these $2n$ vertices consecutively around a new vertex $p_i$ 
in order to get a star-shaped symmetrical graph (compare Figure \ref{f-A.3}). 
Mapping $p_i$ to itself, we have a Hubbard tree.
(Here and elsewhere the degree  \hbox{$d(s)=\w(s)+1$} is copied from the
 scheme.)
All these $s_k$ and $s_k^{\sharp}$ belong to a critical cycle and as such are of
 Fatou type.  Hence, 
the dynamics in this graph is expanding since there is only one Julia type 
vertex in sight (the fixed point $p_i$). 
For future reference we pick a critical vertex in the loop 
(for instance $s_0$, which is critical because it belongs to $|\overline{S}|$
where
$\overline{S}$ is reduced) and call it $c_i$. 
Also, the edge between $c_i$ and $p_i$ will be referred to as $\ell_i$.  

\begin{figure}[!ht]
\centerline{\psfig{figure=milnor-fig14.eps,height=.6in}}
\caption{\it \label{f-A.4} The remaining non-cyclic edges.}
\end{figure}

Let $c_1\,,\,\ldots\,,\,c_m$ be the vertices lying within a critical cycle,
 as numbered above. We now have to perform an extra auxiliary construction. 
Let 
$$c_{m+1}~=~s_{m+1}\,,~\dots\,,~c_{m+r}~=~s_{m+r}~ \in ~\overline{|S|}$$
be the non-periodic critical vertices, i.e, those outside a critical cycle.
For \break \hbox{$i=m+1,\dots, m+r$} consider segments $\ell_i$ between 
$c_i=s_{i}$ and  $s_i^{\sharp}$ (compare Figure~\ref{f-A.4}). 

\begin{figure}[!ht]
\centerline{\psfig{figure=milnor-fig15.eps,height=2.7in}}
\caption{\it \label{f-A.5} Assembling the pieces together. 
Notice that at $c_1$ the angle should be $1/3~({\rm mod}~1)$. 
By construction,
the Julia type fixed points $p_1,~q,~p_2$ $($represented here by 
 circles$)$
have rotation numbers $1/2,~1,~1/4$ respectively. 
Also recall that $F$ maps $c_4^{\sharp}=F(c_4)$ to $c_3$ 
and   $c_3^{\sharp}=F(c_3)$  to $c_1$.}
\end{figure}

Now we are ready to construct the Hubbard tree. 
For \hbox{$i =1,\cdots, m+r$},  add a segment $e_i$ at $s_i$  
making an angle of $1/d(s_i)$ units with $\ell_i$.
(This is to guarantee a complete folding at $s_i$ when we iterate.)
Merge the $e_i$'s at a new vertex $q$ making a uniform angle of $1/(m+r)$ 
between consecutive edges  (the order here is irrelevant). 
Map the Julia vertex $q$ to itself (compare Figure \ref{f-A.5}).
Since there are no adjacent Julia vertices, we have an expanding Hubbard tree. 
 The essentially unique postcritically finite polynomial that realizes
this Hubbard tree, whose existence is guaranteed by Theorem~\ref{t-A1P}, clearly
has the required reduced scheme $\overline S$. 
%Any postcritically finite polynomial that realizes this Hubbard tree clearly 
%delivers the required scheme $S$. 
\end{proof}
\bigskip 














==> milnor-B.tex <==

%\setcounter{table}{0}
\section{Census of Reduced Schemes}\label{sab}

In this appendix, all schemes are to be reduced. The object is to count
the number $N(\w)$ of distinct isomorphism classes of schemes of weight
\hbox{$\w(S)=\w$} for each small value of $\w$. The counting process can be 
broken down  into a number of smaller steps as follows.\bigskip

%Consider only reduced schemes. We want to count the number of
% isomorphism classes of (reduced) schemes of specified total weight.\ms

{\bf (a)\;}~ Every scheme is uniquely a disjoint sum of connected schemes.
If  \hbox{$~S_1 ,~ S_2,~$} \hbox{$~ S_3,~\ldots~$}  is a list of all connected
 schemes,  then every scheme can be expressed uniquely as a sum
$$   S~=~ S_{i(1)} \,+\,S_{i(2)} \,+\,\cdots\,+\,S_{i(k)} \,, $$
where $k$ is the number of connected components, and where 
$$~i(1)~\le~ i(2)~\le~\cdots~\le~ i(k)~.$$
 The total weight of such a sum is \hbox{$~\w(S)=\sum_j \w(S_{i(j)})$}.
Thus, in order to compute the total number $N(\w)$ of schemes of weight $\w$,
it suffices to know the smaller number $N_c(\w')$ of connected schemes of
weight $\w'$, for every $\w'\le \w$. %(Compare paragraph {\bf(4)} below
%for an analogous computation.)  \ednote{\bf ??}
%For small values of $w$,
% details of this computation will be given below.)
\bigskip

%{\bf Definition.} 
\begin{definition}\label{d-tree}
By a \textbf{\textit{~weighted tree~}} will be meant an acyclic simplicial
complex of dimension $\le 1$ with a preferred \textbf{\textit{~root~}} vertex,
together with a weight function which assigns a positive integer to each
non-root vertex. By definition, the root vertex always has weight zero.
The \textbf{\textit{~trivial~}} weighted tree consists of the root vertex alone,
with no edges. \end{definition}

\begin{figure}[!ht]
\centerline{\psfig{figure=milnor-fig16.eps,height=.55in}}
%\vspace{.3cm}
\caption{\it \label{fB1} Splitting off the trees from a scheme of weight
 $~\w(S)=6$.}
\end{figure}

{\bf(b)}~ Every connected scheme $S$ consists of
 a central cycle $C$ of weight\break \hbox{$\w(C)\ge 1$}, together with a
(possibly trivial) weighted 
tree $T(s)$ which is pasted onto each vertex \hbox{$s\in |C|$}.
Here the root point of $T(s)$ is to be identified with $s$.
(Compare Figure~\ref{fB1}, where each root point is represented by the symbol
$*\,$.) Thus
$$ \w(S)~=~\w(C)\,+\,\sum_{s\in|C|} \w\Big(T(s)\Big)\,, \qquad{\rm where}\qquad
\w(T)~=~\sum_{t\in|T|,~t\ne *} \w(t)\,. $$
Note that the cycle $C$ can be economically described by
 a symbol of the form\break
\hbox{$(\w_1,\,\w_2,\,\ldots,\,\w_n)$} which is well defined up to cyclic
 permutation. Here the $\w_i$ are positive integers with sum $\w(C)$. Each 
$\w_i$ corresponds to a vertex $s_i$ of weight $\w_i$ which maps to $s_{i+1}$, 
where the subscript $i$ varies over $\Z/n$.
%The weight of the root point is always set equal to zero when
%computing the total weight of a tree. % forming each
% $w\Big(T(s)\Big)$, since this weight has already been
% counted in $w(C)$.
\bigskip

{\bf(c)}~ By a \textbf{\textit{trunk\/}} of a tree will be meant an edge 
incident to the root
point. Thus every non-trivial tree has at least one trunk. Let
$~T_1,\,T_2,\,T_3,\,\ldots ~$ be a list of all trees with only one trunk.
Then a tree with $k\ge 2$ trunks is isomorphic to a unique wedge sum
\begin{equation}\label{e-ws}
   T~=~T_{i(1)}\,\vee\,\cdots\,\vee\,T_{i(k)}
\end{equation}
 of non-trivial trees pasted together at the root point, where
 $i(1)\le\cdots\le i(k)$. Just as in paragraph
 {\bf(a)} above, the total weight is the
sum $\w(T)=\sum_j \w\big(T_{i(j)}\big)\,.$
(Remember %\ednote{\bf too much\\ repetition}
 that the weight of the root point
 is always zero.)
% For computation of the number of such wedge sums, see {\bf(5)}.
\bigskip

{\bf(d)}~ If $N_{\rm tree}(\w)$ is the number of distinct trees
 of weight $\w$, and  $N_1(\w)$ is the number of such trees with only one trunk,
then %it follows that
\begin{equation}\label{e-sab*}
N_1(\w) ~=~ N_{\rm tree}(0)+N_{\rm tree}(1)+\cdots+
 N_{\rm tree}(\w-1) \,, %~=~N_1(w-1)+N_{\rm tree}(w-1)\,. 
\end{equation}
In fact if $T$ is any tree with just one trunk $T_0\subset T$, then by
collapsing $T_0$ to a point we obtain a tree $T/T_0$ with weight
$$\w(T/T_0)~=~\w(T)~-~\w(T_0)~<~\w(T)\,.$$
 Conversely, $T$ can be reconstructed by pasting
$T/T_0$ onto $T_0$. The identity (\ref{e-sab*}) follows easily.
Note that $N_{\rm tree}(0)=1$, since there is a unique (trivial) tree
 of weight zero.\medskip


%{\bf Proof:} A trunk of any tree of weight $w>0$ can be described as an edge
%%Consider any tree $T$ with just one trunk, consisting of an edge
%$e$ joining a vertex $s$ of weight  $w'\le w$ to the root point. The
%most general tree with only one trunk
% can be obtained, starting with this edge $e$, by pasting the root point of
% an arbitrary tree of weight $w-w'$ onto the vertex $s$. Since there
%are $N_T(w-w')$ such trees, we obtain
%$N_1(w)=\sum_{w'=1}^w N_T(w-w')$, as asserted.\QED
\medskip


\begin{table}[!ht]
\begin{center}
\begin{tabular}{|l|cccccc|}
           \hline
           $\w$ & 0 & 1 & 2 & 3 & 4& 5\cr
           \hline
           $N_1(\w)$ & 0 & 1 & 2 & 5 & 13 & 37\cr
           $N_{\rm tree}(\w)$ & 1 & 1 & 3 & 8& 24& 71\cr
           \hline
\end{tabular}
\vspace{.3cm}
\caption{\it Numbers of trees with given total weight $\w$.\label{tB1}}
\end{center}
\end{table}
The values for $\w\le 5$ are shown in Table~\ref{tB1}.
This table can be constructed inductively as follows. Suppose 
that we know the values
 \hbox{$N_{\rm tree}(\w')$} for $\w'<\w$. Then $N_1(\w)$ can be computed
immediately from equation (\ref{e-sab*}). On the other hand, if we know
\hbox{$N_1(\w')$} for all \hbox{$\w'\le \w$}, then \hbox{$N_{\rm tree}(\w)$} can 
be computed as follows.

 Note that any wedge sum
expression (\ref{e-ws}) gives rise to a partition of the total weight $\w$,
that is a sequence  of positive integers which can be ordered so that

$$ \w(T_{i(1)})~\le~ \w(T_{i(2)})~\le~ \cdots~\le~ \w(T_{i(k)}), $$
with sum   equal to $\w$.
First consider the special case where all $k$ of these wedge summands
have the same weight $\w_0=\w/k$. Then there are $N_1(\w_0)$
possible choices for each of these summands, where their order
doesn't matter. The total number of possibilities in this case is equal to the
binomial coefficient %$ $~ \frac{N_1(w_0)+k-1)!}{k!~N_1(n)-1)!}~.$
\begin{equation}\label{e-bc}
\left(\begin{matrix}
N_1(\w_0)+k-1\\ k
\end{matrix}\right)\,.
\end{equation}
 To see this, let  $a_h$ be the number of
copies of the $h^{\rm th}$ tree in this $k$-fold wedge sum,
so that \hbox{$~a_h\ge 0~$} with \hbox{$~a_1+a_2+\cdots +a_{N_1(\w_0)}~=~k\,$.}
%$$0~\le~ a_1~\le~ a_1+a_2~\le~\cdots~\le~ a_1+a_2+\cdots+ a_{N_1(w_0)}~=~k~,$$
Then the partial sums \hbox{$~a_1+a_2+\cdots+a_i+i~$} with \hbox{$~1\le i<
N_1(\w_0)~$} can be any increasing sequence of \hbox{$N_1(\w_0)-1$} distinct
integers between one and \hbox{$~N_1(\w_0)+k-1$}. Hence the number of
 possibilities is given by the binomial coefficient (\ref{e-bc}).\smallskip

 % $~\left(\begin{matrix}N_1(w_0)+k-1\\ k!~(N_1(w_0)-1)!}
%\end{matrix}\right)$. 
More generally,
suppose that for each $n$ between $1$ and $\w$  there are $~k_n\ge 0~$ summands
of weight $n$, so that
$$ \w~=~ k_1+2\,k_2+\cdots+ \w\,k_\w\,.$$
Then the number of possibilities is equal to the product
$$ \prod_{k_n>0} \left(\begin{matrix}
N_1(n)+k_n-1\\ k_n
\end{matrix}\right)\,,$$
taken over all $n$ with $k_n>0\,.$
Thus, all together, the number of possibilities is given by
\begin{equation}\label{e-tree-ct}
 N_{\rm tree}(\w)~=~\sum_{\rm partitions}~\prod_{k_n>0}
\left(\begin{matrix}
N_1(n)+k_n-1\\ k_n
\end{matrix}\right)\,,
\end{equation}
to be summed over all partitions \hbox{$~\sum n\,k_n\,=\,\w$}.\medskip

As an example, suppose that $N_1(\w)$ is known for \hbox{$\w\le 4$}. Using the
values shown in Table \ref{tB1}, since the 
integer 4 has 5 different partitions
$$ 1+1+1+1~~=~~1+1+2~~=~~1+3~~=~~2+2~~=~~4$$
(using a different notation for partitions),
it follows that \hbox{$~N_{\rm tree}(4)~$} 
 can be expressed as a 5-fold sum
$$\quad\qquad\left(\begin{matrix}4 \\ 4\end{matrix}\right)~+~
 \left(\begin{matrix} 2\\2 \end{matrix}\right)
 \left(\begin{matrix}2 \\ 1\end{matrix}\right)~+~
 \left(\begin{matrix}1 \\1 \end{matrix}\right)
 \left(\begin{matrix}5 \\ 1\end{matrix}\right)~+~
% \left(\begin{matrix}1 \\1 \end{matrix}\right)
 \left(\begin{matrix}3 \\ 2\end{matrix}\right)~+~
 %\left(\begin{matrix}1 \\1 \end{matrix}\right)
 \left(\begin{matrix}13 \\ 1\end{matrix}\right)
% \left(\begin{matrix}2 \\1 \end{matrix}\right)
% \left(\begin{matrix}5 \\ 1\end{matrix}\right)~+~
% \left(\begin{matrix}37 \\ 1\end{matrix}\right)
\,,$$
yielding $$~N_{\rm tree}(4)~=~1+2+5+3+13~=~24\,.$$ Other entries in
Table \ref{tB1} can be computed similarly.
\bigskip

The following table lists the 
number of connected schemes for each given value of the cyclic weight $\w(C)$
together with the tree weight $\sum_{s\in|C|} \w(T(s))$, within the range
 \hbox{$~\w(S)\,=\,\w(C) + \sum \w(T)\,\le\, 6$}. % \ednote{\bf Check entries}

\begin{table}[!ht]
\begin{center}
\begin{tabular}{cc|cccccc|c|}
%\cline{3-8} 
%& &\multicolumn{6}{|c|}{$\sum w(T)=\!\!\!$} \\ \cline{3-8}
\hline
\multicolumn{2}{|c|}{$\sum \w(T)=\!\!\!$}& 0 & 1 & 2 & 3 & 4 &5\\ %\cline{1-8}
\hline
\multicolumn{1}{|c|}{\multirow{6}{*}{$\w(C)=$}} &
\multicolumn{1}{|c|}{1} & 1 & 1 & 3 & 8 & 24 & 71   \\ %\cline{2-7}
\multicolumn{1}{|c|}{}                        &
\multicolumn{1}{|c|}{2} &  2 & 2& 7 & 19&62&  \\ %\cline{2-7}
\multicolumn{1}{|c|}{}                       &
\multicolumn{1}{|c|}{3} & 3 & 4 & \underline{14} &45& & \\ %\cline{2-7}
\multicolumn{1}{|c|}{}                        &
\multicolumn{1}{|c|}{4} & 5 & 8& 31 & & &\\ %\cline{2-7}
\multicolumn{1}{|c|}{}                        &
\multicolumn{1}{|c|}{5} & 7 &16& & & &\\ %\cline{2-7}
\multicolumn{1}{|c|}{}                        &
\multicolumn{1}{|c|}{6}& 13& & & & &\\ \cline{1-8}
\end{tabular}
\vspace{.3cm}
\caption{\it Number of connected schemes $S$ with given $\w(C)$ and 
$\sum \w(T)$. %, and with sum $~w(S)\,=\,w(C)+\sum w(T)\,\le\, 6$.
\label{tB2}}
\end{center}
\end{table}


 Rather than explaining each entry in this table, let me simply give a detailed
explanation for the one typical entry which is underlined in the table,
 corresponding to cyclic weight
\hbox{$\w(C)=3$},~ tree weight \hbox{$\sum \w(T)=2$},~ and hence total weight 
\hbox{$3+2=5$}.
 For this example,  we need to know the numbers
\hbox{$N_{\rm tree}(1)=1$} and \hbox{$N_{\rm tree}(2)=3$}, and we need to study
 each of the three cyclic
schemes of weight \hbox{$\w(C)=3$} separately. Here are the three cases, with
 notation as in {\bf(b)} above.

\begin{itemize}
\item For the cycle $(3)$, with a single vertex of weight 3, we can paste
any one of the three trees of weight 2 onto the unique cyclic vertex,
 so we get a total of 3 possible schemes.\medskip

\item  For the cycle $(1,2)$, we can paste a tree of weight 2
 onto either one of the two vertices, yielding 6 distinct possibilities.
 But we can also paste a  tree of weight one onto each vertex, yielding a
 7-th possibility.\medskip

\item For the cycle $(1,1,1)$, note that there is a cyclic group of
 symmetries. Again we can paste a tree of weight 2 onto any vertex, but
because of the symmetries, it doesn't matter which vertex we choose, so
 there are three distinct possibilities.
Similarly, we can paste a tree of weight one onto each of two vertices,
yielding a 4-th possibility. (Again, because of the symmetries,
it doesn't matter which two we choose.)
\end{itemize}
\smallskip

\noindent Thus, all together, we get $~3+7+4=14~$
 distinct schemes, as listed in Table \ref{tB2}. Other entries in this
table can be computed similarly.\bigskip

%(Care is needed here, since many cyclic schemes have cyclic
%symmetries, which reduce the number of distinct schemes obtained
%by this construction. As an example, if we rotate the scheme of Figure B.1
%by $180^\circ$, then we obtain a scheme which is isomorphic, but described in
%a slightly different way.)

The number $N_{\rm c}(\w)$ of connected schemes of weight
$\w$ can be obtained by adding entries along the diagonal 
\hbox{$~\w(C)+\sum \w(T)=\w~$}
in Table~\ref{tB2}. For example
$$  N_{\rm c}(5)~=~ 7+8+14+19+24~=~72\,.$$
For $n\le 6$, the total number $N_{\rm c}(\w)$  of connected
schemes of  weight $\w$, computed in this way,
 is listed in the middle row of Table~\ref{tB3}.
The total number $N(\w)$ of all schemes, connected or not, can then be computed
by a formula completely analogous to (\ref{e-tree-ct}) above,
%that used to justify Table~\ref{tB1},
and is listed in the last row below (as well as in Table \ref{t-numbers}).

\begin{table}[!ht]
\begin{center}
\begin{tabular}{|l|cccccc|}
           \hline
           $\w$  & 1 & 2 & 3 & 4& 5 &6\cr
\hline
           $N_{\rm c}(\w)$ & 1 & 3 & 8 & 24 & 72 & 238\cr
           $N(\w)$ & 1 & 4 & 12 & 42& 138& 494\cr
\hline
\end{tabular}
\vspace{.3cm}
\caption{\it The total count.\label{tB3}}\end{center}
\end{table}





